Language-agnostic Multilingual Modeling

Multilingual Automated Speech Recognition (ASR) systems allow for the joint training of data-rich and data-scarce languages in a single model. This enables data and parameter sharing across languages, which is especially beneficial for the data-scarce languages. However, most state-of-the-art multilingual models require the encoding of language information and therefore are not as flexible or scalable when expanding to newer languages. Language-independent multilingual models help to address this issue, and are also better suited for multicultural societies where several languages are frequently used together (but often rendered with different writing systems). In this paper, we propose a new approach to building a language-agnostic multilingual ASR system which transforms all languages to one writing system through a many-to-one transliteration transducer. Thus, similar sounding acoustics are mapped to a single, canonical target sequence of graphemes, effectively separating the modeling and rendering problems. We show with four Indic languages, namely, Hindi, Bengali, Tamil and Kannada, that the language-agnostic multilingual model achieves up to 10% relative reduction in Word Error Rate (WER) over a language-dependent multilingual model.

==> data_description.tex <==
\section{Data Description}
\label{sec:dataDescrciption}

The training and test data for the four Indic languages consist of anonymized, human-transcribed utterances representative of Google's voice search traffic described in~\cite{kannan2019large, datta_kanna_2019}. Of the four languages, Hindi, Bengali, Tamil and Kannada, Hindi has the most amount of training data and Kannada has nearly two orders of magnitude less training data than Hindi, with Tamil and Bengali falling in between. The training data is augmented with additional copies from noisy utterances created by corrupting the utterances using a room simulator \cite{Chanwoo17} and noise styles as described in section \ref{ssec:data_balancing}.


% While the amount of training data roughly correlates to the availability of transcribed data in each languages, we have reduced the data amount for Kannada (~1K hours) to further increase the data skew, as we were particularly interested in addressing the challenge of data imbalance. 

%Transcript for training (before transliteration) and test data for a language were in the native script with a few Latin-case English words.   

% \begin{table}[!t]
% \centering
% \begin{tabular}{|c|c c|} \hline
% Language      & Train             & Test  \\
%               & \# utts (\# hours) & \# utts  \\\hline
% Hindi (Hi)    &  15.7M (17.6K)     & 6.3K \\
% Bengali (Bn)  &  3.9M (4.5K)       & 3.6K \\
% Tamil (Ta)    &  1.8M (1.9K)       & 5.5K \\
% Kannada (Kn)  &  200K (211)       & 1.1K \\ \hline
% \end{tabular}
% \caption{Training and Test data sets.}
% \label{table:data}
% \vspace{-0.2 in}
% \end{table}


